An Approximate Dynamic Programming Framework for Occlusion-Robust Multi-Object Tracking

In this work, we consider data association problems involving multi-object tracking (MOT). In particular, we address the challenges arising from object occlusions. We propose a framework called approximate dynamic programming track (ADPTrack), which applies dynamic programming principles to improve an existing method called the base heuristic. Given a set of tracks and the next target frame, the base heuristic extends the tracks by matching them to the objects of this target frame directly. In contrast, ADPTrack first processes a few subsequent frames and applies the base heuristic starting from the next target frame to obtain tentative tracks. It then leverages the tentative tracks to match the objects of the target frame. This tends to reduce the occlusion-based errors and leads to an improvement over the base heuristic. When tested on the MOT17 video dataset, the proposed method demonstrates a 0.7% improvement in the association accuracy (IDF1 metric) over a state-of-the-art method that is used as the base heuristic. It also obtains improvements with respect to all the other standard metrics. Empirically, we found that the improvements are particularly pronounced in scenarios where the video data is obtained by fixed-position cameras.

==> recycle.tex <==
In this work, we consider the problem of multi-object tracking (MOT). In particular, we address the challenges arising from object occlusions.
We propose a solution based on a principled approximate dynamic programming approach called \textit{ADPTrack}. ADPTrack relies on existing MOT solutions and directly improves them.
When matching tracks to objects at a particular frame, the proposed approach simulates executions of these existing solutions into future frames to obtain approximate track extensions from which a comparison of past and future appearance feature information is leveraged to improve overall robustness to occlusion-based error.
When applied to the MOT17 dataset, the proposed solution demonstrates a 0.7\% improvement in the association accuracy (IDF1 metric) over a state-of-the-art method that is used as a base heuristic. It also obtains improvements with respect to all other metrics.
Empirically, we found that this improvement is even more pronounced in scenarios where the camera maintains a fixed position. 
% This implies that the proposed method is effective in addressing MOT issues pertaining to object occlusions.
**************************************************************************************************
In this work, we consider the problem of \textit{multi-object tracking} (MOT), which can be viewed as a special case of the multidimensional assignment problem~\cite{emami}. It involves the assignment of identifiers to objects in motion over a sequence of image frames. 
However, the task of ensuring a consistent assignment remains a formidable challenge. In particular, for scenarios where objects become occluded, where shadows temporally affect the illumination of objects, where the objects themselves alter in appearance, or in the presence of sensor error.
To overcome the occlusion challenge, we introduce a method based on approximate dynamic programming (also known as reinforcement learning) techniques that improves over an arbitrary online tracking algorithm. Online tracking algorithms match frame-to-frame and do not use any subsequent frames' information while matching the current frames. We move the online tracking algorithm to a near-online (i.e., considering a limited amount of future information) setting, where we use a near-online simulation of subsequent frames and appearance feature comparison of past and future frames.
We argue that our more principled approach dramatically reduces error caused by occlusions---namely, identifier swaps, i.e., erroneous assignment of identifiers while maintaining the overall accuracy of existing state-of-the-art solutions. 

Many existing state-of-the-art methods for online tracking employ an \textit{object detection module} and a \textit{tracking module}~\cite{bytetrack, botsort, cbiou, corrtracker, p3aformer, strongsort, motiontrack, stam, sgt, utm}. 
The object-detection module involves the computing of bounding boxes for objects in the frame. The tracking module involves a motion model (e.g. a constant velocity Kalman filter~\cite{sort}) for state estimation, an appearance model (e.g. a re-identification\footnote[1]{Appearance features of an object calculated from the image patch of its bounding box} neural network~\cite{fastreid}) for calculating appearance similarities, and a matching algorithm to match the bounding boxes over different frames.
Note that at any given frame there may not exist a bijection of tracks to objects, as some objects may disappear or new objects may appear suddenly.
In recent publications, there has been a considerable improvement in the methodology used for object detection~\cite{yolox, yolov7, faster}. % and re-identification~\cite{botsort, fastreid, fairmot}.
However, there has been a lack of focus on effectively using subsequent frames to match the current frames. 
As such, this work presents a methodology for applying existing online
state-of-the-art multi-object tracking methods that comprise motion and appearance models as a base heuristic for a reinforcement learning technique called \textit{approximation in value space}~\cite{bertsekas2023course} with the aim to better associate occluded objects through information obtained from online simulations.

In this work, we offer a key insight for improved multi-object tracking: 
Namely that, MOT has an intuitive dynamic programming structure (discussed in Section~\ref{sec:preliminaries}). Although the problem is difficult to solve exactly, it brings to bear existing approximate dynamic programming techniques for near-optimal solutions of MOT.
In particular, approximation in value space is a technique used to approximate the cost-to-go terms of the Bellman equations, and these approximations frequently involve online simulation to compute approximately optimal costs for smaller subproblems.
Approximation in value space has substantial theoretical support, which suggests that it may be a promising candidate method for MOT.
We demonstrate empirically that an approximation approach using simulation renders existing methods more robust to object occlusions, and therefore may supplement any arbitrary state-of-the-art method.
Specifically, we present an MOT tracking algorithm for near-online motion model and appearance feature-based 
tracking called \textit{ADPTrack}, where ADP refers to approximate dynamic programming.
%In our experiments, we equip ADPTrack with BoT-SORT~\cite{botsort}---one of the current state-of-the-art for online MOT at the time of writing.
In our experiments, we equip ADPTrack with one of the current state-of-the-art online MOT algorithms at the time of writing---BoT-SORT~\cite{botsort}, as a base heuristic.
We tested our solution on the MOT17~\cite{milan2016mot16} dataset and observed an overall relative improvement of 0.7\% in the IDF1 score metric over BoT-SORT with a minor improvement in accuracy (MOTA, HOTA metrics).
This implies ADPTrack is useful for reducing false positives, false negatives, ID switches, and fragmentation with respect to the ground truth, and may be applied to any existing method that uses motion models and appearance features.
Figure~\ref{fig:main-example} provides a frame-by-frame comparison of BoT-SORT and ADPTrack with a BoT-SORT heuristic for a fixed video example and illustrates occlusion scenarios where ADPTrack improves over existing solutions.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{Styles/000089cropped.jpg}
        \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{Styles/000099cropped.jpg}
        \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{Styles/000106cropped.jpg}
        \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{Styles/000112cropped.jpg}
        \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{Styles/000089adp.jpg}
        \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{Styles/000099adp.jpg}
        \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{Styles/000106adp.jpg}
        \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.22\textwidth}
        \includegraphics[width=\textwidth]{Styles/000112adp.jpg}
        \caption{}
    \end{subfigure}
    \caption{Frame-by-frame comparison of BoT-SORT-Reid (a-d) versus ADPTrack with BoT-SORT-Reid heuristic (e-h) for a fixed video example. With BoT-SORT-Reid alone, person 6 occludes person 4, which causes 4 to be erroneously assigned another person's identifier (14) located between person (4) and person (9). With ADPTrack based on BoT-SORT, the same person (here identified with identifier 16) occludes person 4 without an identifier switch.}
    \label{fig:main-example}
\end{figure}

***************************************************************************

Existing literature in MOT can be classified into four areas: online, near-online, batch, and offline tracking. 
Online tracking matches objects present in adjacent frames by using accumulated information from assigned previous frames. 
Specifically, at any time $k+1$, the online tracking methods perform matching only between the tracks generated to time $k$ and objects at frame $k+1$.
% Note that this does not use information from subsequent frames, and as such, the algorithms proposed in this area are considerably faster. 
Online trackers typically consist of motion and appearance models, and a matching algorithm. 
The state at time $k + 1$ would consist of existing tracks at time $k$ and new detections at time $k$. 
A motion model performs a state estimation of each track for the next time step. 
This information is compared to the new detections at time $t$ using a localization scoring metric to obtain the distance between the new and estimated objects. 
An appearance model is used to compute similarity scores between the tracks and the new detections based on appearance.
The information from one or both of these models is used to produce a pairwise similarity score between each existing track and new detection. 
The pairwise similarity scores are computed between the existing tracks and the new detections, and all this data is represented as a cost matrix.
An optimal minimum cost bipartite matching algorithm (e.g. Hungarian algorithm~\cite{sort}) or a greedy algorithm is generally applied to the cost matrix.
It is used to extend the existing tracks by one further frame.
% Any unmatched tracks may be maintained for some frames (typically given as a parameter) before being discarded, whereas new objects initiate new tracks.

% We first discuss online tracking methods that involve a motion model. Then, we explore tracking algorithms that use an appearance model to match objects based on appearance features. Lastly, we discuss approaches that use a set of previously matched objects from a track to match a new object.
% We provide an overview of the state-of-the-art MOT algorithms and focus on literature that most closely relates to our solution.
% In particular, we contrast our approach with existing near-online and reinforcement learning-based solutions, as our work relates most closely with this intersection.
% In this section, we provide an overview of the existing approaches to online tracking.

Many state-of-the-art papers have shown the importance of a motion model, especially in the case of a fast-moving camera~\cite{botsort, strongsort, tracktor}. A motion model is used to estimate the position and size of an object in the next state using the velocity of the object. An object's velocity (which we refer to from here onward as \textit{motion cues}), position, and size are used to calculate an association cost with a new object using distance metrics.
In~\cite{sort, bytetrack, botsort, deepsort}, a Kalman filter with a linear-constant velocity model is used for state estimation.
%, and \textit{intersection over union overlap} (IOU overlap) between the predicted bounding box and the detections is used in the estimation of the cost-matrix that is used for an optimal association using Hungarian algorithm or greedy assignment. 
% In~\cite{deepsort}, the motion affinity is estimated by calculating Mahalanobis distance between the estimated state and the new detections.
In~\cite{ocsort}, the authors re-update the Kalman filter parameters and predictions after a lost track is matched again by constructing a virtual trajectory between the previously found detection and the newly matched detection. 
In \cite{strongsort}, the authors use the Noise-Scale-Adaptive (NSA) Kalman filter~\cite{nsakalman} where the detection confidence score weights the update step.
In~\cite{cbiou}, a linear combination of limited previous frames is used to account for a change in the object's direction or motion.
In~\cite{motiontrack}, the authors have an interaction module to calculate interactions between existing tracks and update the next state of every track accordingly using a graph convolution module.
In~\cite{iou, viou}, the authors do not use an explicit motion model to estimate the next state. They make an assumption that detections in consecutive frames would have a high overlap.
% In~\cite{viou}, the authors use a visual tracker to track the lost tracks for a few frames forward and backward in time, to check and merge the newly generated tracks with their original tracks.
In~\cite{tracktor}, the authors use bounding box regression between the detections to track objects.
Similar to these methods, our method also relies on a base heuristic with a motion model to specifically help match objects that are mostly occluded during occlusion.

Several state-of-the-art (SOTA) leverage appearance features of the objects~\cite{botsort, corrtracker, p3aformer, cstrack, stam, utm, conf, poi} to perform association.
In~\cite{siamese1, siamese2, siamese4, dan, uma}, deep neural networks are used to obtain similarity costs between image patches of bounding boxes.
%In~\cite{deepsort}, the authors compute a cosine distance between the appearance features generated by a deep neural network as trained by the authors on a re-identification dataset and fuse both the motion affinity and the appearance scores. 
In~\cite{deepsort, motdt, jde, fairmot}, the authors use a distance metric to compute the similarity between the appearance features generated by a deep neural network.
% In~\cite{motdt}, the authors use a scoring function based on image classification to obtain candidate tracks and then perform hierarchical association by using appearance features-based similarity scoring on the first set of tracks, and only IOU overlap for the second set of tracks. 
% In~\cite{jde, fairmot}, the authors train a neural network to jointly learn and infer detections as well as embeddings for appearance features. 
% In~\cite{jde}, the authors propose smoothing the representative appearance features of the track with the new detection features using an exponential moving average after a match has been identified between the existing track and the corresponding new detection. 
%In~\cite{siamese1, siamese2, siamese4, dan, uma}, deep neural networks are used to obtain similarity costs between image patches of bounding boxes of the current frame and next frame detections, which are used to perform associations, without the usage of any motion model for state estimation.  
In~\cite{botsort}, appearance feature similarity scores are fused with IOU overlap scores to get association costs.
We are using the BoT-SORT algorithm as a baseline for our work. Solutions that focus on track histories demonstrate the importance of considering past frame features while matching objects in the current frame.
These proposed solutions were given in~\cite{ran, ttu, strn, siamese3, lsst, soda, dman,  transtrack, transmot, tadam,  trackformer, utt, memot, tpagt, quasidense}, where the previous frame features are passed in conjunction as input to a deep neural network such as a CNN, RNN, or a transformer to obtain pairwise similarity scores of the existing tracks and the new detections. 
While this is not how we use the past frame features in our method, these papers demonstrate the importance of the past frame features during association. 



%\subsection{Near-online Tracking}
Near-online tracking is similar to online tracking, where the tracker (i.e., a tracking algorithm) matches the tracks generated until time $k$ to objects at a frame $k+1$, where only two frames are matched and the algorithm proceeds sequentially temporally. However, the tracker uses information from the past as well as a limited amount of subsequent frames'. 
%Near-online tracking consists of methods that consider a limited number of future and possibly past frames. 
% As the near-online tracking methods consider a limited number of future frames, say $\ell$, while matching the current frames $k$ and $k+1$, there is a certain lag (of at least $\ell$ frames) associated with this type of algorithms. 
% This lag places the camera input at $k+\ell+2$th (or further) frame while processing the matching between frames $k$ and $k+1$. 
% There may also be a certain lag associated with the computation of the matching between the frames $k$ and $k+1$.
% Overall, these algorithms may not be as fast as online tracking algorithms, but this compromise in real-time tracking is seen as a trade-off for improved tracking accuracy.
%In~\cite{nomt1}, the authors introduce the concept of near-online multi-object tracking. They construct a future trajectory for every detection by using a flow descriptor, i.e. a heuristic used to assess the likelihood that two temporally distant objects represent the same object. These future trajectories are used to obtain the association between the current frames using a graphical model (conditional random field).
%In~\cite{nomt1}, the authors introduce the concept of near-online multi-object tracking. They construct a future trajectory for every detection by using a flow descriptor, i.e. a heuristic used to assess the likelihood that two temporally distant objects represent the same object. These future trajectories are used to obtain the association between the current frames using a graphical model (conditional random field).
In~\cite{nomt1}, the authors introduce the concept of near-online multi-object tracking. They construct future trajectories using a flow descriptor and perform an association using a graphical model.
In~\cite{nomt2}, the future tracks are generated by greedy associations using only appearance features. Association is then performed with costs gnenerated by three neural networks.
% Then three neural networks are used to generate similarity scores between tracks at a time $k$ and new detections at time $k+1$. 
% These neural networks compare tracks at time $k$ to detections at $k+1$, as well as the track histories of tracks at $k$ to detections at $k+1$, as well as track histories to track hypotheses.
% Once the costs are generated, a greedy association is performed.
In~\cite{nomt3}, the authors present a novel way of handling appearance features using body and joint detections, and the association optimization is modeled as a minimum-cost graph labeling problem. 
A similar graph labeling approach that ranks trajectories was used in~\cite{multiplex}.
Moreover, in~\cite{flow}, the authors compartmentalize the problem locally around a time window using a network construction technique, which is then solved as if it were the full problem using multicommodity flow-based optimization techniques.
In~\cite{trackmpnn}, the authors perform a near-online data association directly using graph neural networks.
In~\cite{MCMC}, the authors use a statistical physics approach for approximately optimal data association over a sliding window of frames. 
In contrast, our approach focuses on improvement over an online base heuristic. 
We simulate the base heuristic equipped with both motion and appearance models over a limited set of subsequent frames to generate tracklets. 
We may then leverage any appearance feature association method given by the base heuristic, as well as information from future tracks as generated by the base heuristic.
As such, our approach differs from the methods listed here in that it focuses on improving existing solutions via online simulation.

Batch tracking matches a set of frames simultaneously using information available from every frame.
Offline tracking can be viewed as a special case of batch tracking where the batch consists of the entire frame sequence.
Multi-hypothesis tracking~\cite{mht} maintains a collection of tree topologies representing track hypotheses. 
Several extensions of this method~\cite{mhtr, tlmht, edmt, bilstmmht} introduce pruning and propose hypothesis-scoring techniques.
In \cite{multicut}, the multi-object tracking problem is formulated as a minimum-cost multicut problem. 
Other methods perform end-end data association using neural networks~\cite{dnf, famnet, gtt, mpntracker}.
Other offline solutions include~\cite{gogm, lifm, graphfusion, fusion}.

%\subsection{Reinforcement Learning-based Multi-object Tracking}
In~\cite{asmot}, the authors formulate the multi-object tracking and segmentation problem as a dynamic programming problem by considering costs for each matching and costs across temporally adjacent matchings. 
%It is a batch method where they consider a set of frames to be matched at once. At any time $k$, they consider a limited number of best matches between the detections of time $k$ and time $k+1$ using the Hungarian-Murty algorithm~\cite{hungarianmurty}. Here the cost of a matching is the sum of the total associations made in that matching, which is driven by IOU overlap and appearance similarities. They formulate a cost between the temporally adjacent matches to construct the cost of a total trajectory. The optimal cost is then obtained by solving it through dynamic programming. In~\cite{learningtotrack}, the track's state is formulated as a policy that is decided by a Markov decision process that learns the association cost while learning the policy. 
In~\cite{marl1, marl2}, the multi-object tracking problem is formulated as a multi-agent reinforcement learning problem, where data association between two frames is equivalent to joint policies taken by all the agents. %Deep reinforcement learning models such as Trust Region Policy Optimization (TRPO) and Q-learning are trained on the ground-truth data to learn the joint actions. 
In~\cite{marl3}, a prediction and a decision network are trained to predict the detections in the next frame using the current tracks and decide a policy for the tracks and detections in a multi-agent environment according to the valid actions present, respectively.
In contrast to these approaches, we introduce approximations to the Bellman equations based on the results of online simulation of heuristics.

% \subsection{Road Map}
% In section~\ref{sec:preliminaries}, we present preliminary materials, including a formal description of MOT as a special case of the multidimensional assignment problem, as well as an overview of approximation in value space.
% In section~\ref{sec:algorithm}, we present the ADPTrack algorithm and its technical specifications.
% In section~\ref{sec:experimentalstudy}, we present an experimental study that applies ADPTrack to the MOT17 dataset.
% Lastly, in section~\ref{sec:discussion}, we discuss the implications of our findings as well as avenues for future research.


******************************************************************************
We consider a DP approach since such frameworks admit straightforward approximations. We first describe a DP formulation for the multi-dimensional assignment problem, and then describe a technique called \textit{approximation in value space}, which forms the foundation of our proposed algorithm in Section~\ref{sec:algorithm}. For a dynamic programming framework, we require four objects: a state space $\Omega$; a state-dependent control space $U(x)$; a system equation $x'=f(x,u)$ where $x,x'\in\Omega$ and $u\in U(x)$; and a cost function $G(\cdot)$.
We frame the problem as a sequential decision problem where at each layer $\mathcal{N}_k$, we choose a perfect matching of cardinality $m$ to the nodes of layer $\mathcal{N}_{k+1}$.
The control space $U_k(x_k)$ at state $x_k$ is the set of all perfect matchings between layer $\mathcal{N}_k$ and $\mathcal{N}_{k+1}$.
The state space is the set of all partial sequences of perfect matchings between consecutive layers up to layer $k$, for $k=0,1,\ldots,N-1$.
As such, a state $x_k\in\Omega$ consists of a particular set of perfect matchings between layers $\mathcal{N}_{\ell}$ and $\mathcal{N}_{\ell+1}$, for all $\ell=0,1,\ldots, k-1$, and can be expressed as a sequence of controls $x_k=(u_0,\ldots,u_{k-1})$.
The system equation $x_{k+1}=f(x_k,u_k)=(x_k,u_k)$ extends the sequence of perfect matchings by one, and the cost function $G(x_N)=G(u_0,\ldots,u_{N-1})$ applies to a complete grouping set (i.e. $m$ groups of $N+1$ nodes).
The exact dynamic programming algorithm to determine the cost $J_k^*(x_k)$ of an optimal sequence of perfect matchings beginning at layer $\mathcal{N}_k$ is given by the Bellman equations and takes the form:
   $$ J^*_N(x_N)=G(x_N)=G(u_0,\ldots,u_{N-1}),$$
and
\begin{equation}\label{eq:bellman}
    J^*_k(x_k)=\min_{u_k\in U_k(x_k)}J^*_{k+1}(x_k,u_k), \hspace{8mm} \text{for all }x_k,k=0,\ldots,N-1
\end{equation}

Three major issues arise when attempting to compute $J^*_k(\cdot)$.
The first applies specifically to the problems of data association and multi-object tracking, namely that evaluating the quality of a matching sequence is difficult and cost function $G(\cdot)$ is not known. 
Secondly, the size of the control space per state corresponds to the number of perfect matchings on bipartite graph, of which there may be exponentially many.
Lastly, even if $G(\cdot)$ were known and the control space polynomial in size, computing $J^*_{k+1}(\cdot)$ is still intractable.
To address these challenges, we resort to a broad technique called \textit{approximation in value space}, which introduces various approximations to the components of the Bellman equations.
One such approximation replaces $J^*_{k+1}(\cdot)$ with an approximation given by $\tilde{J}_{k+1}(\cdot)$ that can be computed efficiently.
To address the remaining two challenges, $\tilde{J}_{k+1}(\cdot)$ is granted a special structure suitable for the use of fast 2-dimensional assignment algorithms.
Namely, 
\begin{equation}\label{eq:kplus1tilde}
    \tilde{J}_{k+1}(x_k,u_k)=\sum_{(i,j)\in u_k}c_{k+1}^{ij}(x_k)
\end{equation}
where each $(i,j)\in u_k$ is an arc from the valid perfect matching specified by control $u_k$, and $c_{k+1}^{ij}(x_k)$ represents the cost for arc $(i,j)$ where $i\in\mathcal{N}_k$ and $j\in \mathcal{N}_{k+1}$.
In the case of multi-object tracking, these costs are generated from heuristics, sensor data, and assignments in previous layers.
To handle the large control spaces, costs for all possible pair-wise arcs between layers $\mathcal{N}_k$ and $\mathcal{N}_{k+1}$ are generated and an algorithm for weighted matching online is applied to extract a control.
The cost of an approximately optimal sequence of matchings beginning at layer $\mathcal{N}_k$ is then given by
\begin{equation}\label{eq:approxbellman}
    \min_{u_k\in U_k(x_k)}\tilde{J}_{k+1}(x_k,u_k),\hspace{8mm}\text{for all }x_k,
\end{equation}
which can be computed efficiently as the problem is reduced to a sequence of $N$ 2-dimensional weighted bipartite matching problems.


************************************************************

Existing near-online methods solve the matching of the target frame with the given tracks as a sub-problem of multi-frame matching or use heuristics solely based on appearance features for constructing the tentative tracks. 
However, in ADPTrack, we provide a framework for systematically improving any arbitrary online tracking method that employs motion and appearance models by shifting it to a near-online setting through approximation in value space. 
In particular, approximation in value space is a technique used to approximate the cost-to-go terms of the Bellman equations, and these approximations frequently involve online simulation to compute approximately optimal costs for smaller subproblems. 
The online tracking method is used as a base heuristic in our framework and is used to generate tentative tracks by simulation.
Using a base heuristic with both motion and appearance models ensures the correct matching of objects under occlusion during simulation. 
The tentative tracks in conjunction with the existing tracks are used to match the target frame with the given tracks through visual correspondence. 

***************************************************************
In this section, we describe our proposed algorithm called \textit{Approximate Dynamic Programming Track} (ADPTrack).
Our proposed solution aims to compute~\ref{eq:approxbellman}, and our methodology generates the costs from Equation~\ref{eq:kplus1tilde} using online simulation of a base heuristic over future frames as well as past information through appearance feature-based methodology prescribed by the base heuristic.
To further improve online efficiency, we impose a \textit{truncated horizon}, meaning online simulations are limited to $\ell$ frames into the future. 
We present an illustration of approximation in value space as applied to the multi-dimensional assignment problem in Figure~\ref{fig:alg} (a).

\begin{figure}
\centering
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Styles/alg_color.pdf}
    \label{fig:copy-yuchao}
    \caption{}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=0.6\textwidth]{Styles/nearonlinesim_color.pdf}
    \label{fig:nearonline}
    \caption{}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Styles/costfuncapprox_color.pdf}
    \label{fig:costfuncapprox}
    \caption{}
\end{subfigure}
\caption{(a) Visualization of approximation in value space applied to the multi-dimensional assignment problem. The red layers represent those included in partial groupings up to time $k$. The cost function approximation $\tilde{J}_{k+1}(\cdot)$ is dependent on a cost matrix $c_{k+1}$, which is computed using information obtained from a truncated horizon of length $\ell$ (blue and orange layers).
    We select a minimum weight perfect bipartite matching $u_k$ at time $k$ applied to $c_{k+1}$. (b) Visualization of near-online simulation in ADPTrack. A tracking simulation is performed for a truncated horizon ($\ell$ frames) using a base heuristic with a motion model. The base heuristic is initialized at time $k+1$ for the simulation. (c) Visualization of cost matrix approximation in ADPTrack. Consider the arc between the first track at frame $k$ and the second detection at frame $k+1$. To calculate the cost value $c^{12}_{k+1}$, unlike the base heuristic (online tracker) that compares the track at frame $k$ to the detection at frame $k+1$, we compare the track at frame $k$ to the tracklet starting at frame $k+1$ generated by the near-online simulation. The comparison is performed by pairwise appearance features similarity computations (Equation \ref{eq:prev_future_score}).}
\label{fig:alg}
\end{figure} 

ADPTrack can be categorized as a near-online tracking method where we first simulate the base heuristic for a limited number of subsequent frames from $k+1$ to $k+\ell+1$. 
Next, we augment the cost matrix between existing tracks at $k$ and detections at $k + 1$ using the tracklets generated via simulation. 
Similar to the general near-online methods, we perform the association between frames $k$ and $k+1$ by considering a temporal window from frame $k$ to frame $k +\ell+1$ by following a sliding-window concept, where the window shifts one time-step forward after each association.
ADPTrack comprises two components: Near-online simulation, and cost-matrix augmentation \& matching.

\subsection{Near-online Simulation}\label{nearonline-sim}
Given a base heuristic that is an online tracking algorithm based on a motion model (and may also exploit an appearance feature model), we simulate $\ell$ frames starting from frame $k+1$ and generate \textit{tracklets} (i.e. tracks of limited length) until frame $k + \ell + 1$. 
In this context, simulation implies using the base heuristic to sequentially match consecutive frames from time $k+1$ to $k + \ell + 1$. 
An illustration is presented in Figure~\ref{fig:alg} (b).
Conceptually, we assume that objects that become occluded have similar appearance features before and after the occlusion, and also similar motion cues.
This motivates the method of near-online simulation to produce future tracklets, which can then be compared with the past when determining associations.
For this simulation, we choose base heuristics grounded in motion models (or at least that incorporate localization information by using position and size properties between detections of adjacent frames), as the appearance features of an object are not informative when the object is mostly occluded, and hence a motion model can provide better estimations in such scenarios.
Note that the appearance features become valuable again when the object becomes partially visible again.
How the appearance features of the generated tracklets are used for matching the current frames $k$ and $k+1$ is explained in the next section.

At the beginning of the near-online simulation, a motion model adopted by the base heuristic is initialized at frame $k+1$ for each tracklet starting at frame $k+1$, and considers no information on the past frames until $k$. 
The motion model is then updated as a result of associations of detections in frames $k+1$ to $k + \ell + 1$. 
For object $j$, a tracklet generated by near-online simulation starting at time $k+1$ is represented by $t^j_{k+1}$.
During the execution of the simulation, we follow the same motion model policies, appearance features-based score calculations (if present in the base heuristic), track-management policies, and any other additional components involved that are prescribed by the base heuristic.

\subsection{Cost-matrix Augmentation and Matching}\label{section:costvalues}
In this section, we discuss how the tracklets generated by near-online simulation are used for matching a frame $k$ to $k+1$. 
We describe how to generate a cost matrix $c_{k+1}$ (corresponding to Equation~\ref{eq:kplus1tilde}), which is expressed as a convex combination of two matrices $c'_{k+1}$ and $c''_{k+1}$.
At a high level, $c'_{k+1}$ is a matrix whose entries are based on comparisons (both appearance feature and motion-based) between the tracks until frame $k$ and new bounding boxes are generated at frame $k+1$.
On the other hand, $c_{k+1}''$ contains costs that represent relationships between past and future information (i.e. frames beyond $k+1$) with respect to appearance features \textbf{only}.
As such, $c_{k+1}$ is a cost matrix that temporally aggregates appearance features in both the past and the future, and also accounts for motion cues in the present.
More weight applied to $c_{k+1}'$ implies that the information extracted from the current frame $k+1$ is more relevant to the costs, whereas more weight to $c_{k+1}''$ implies that future information is more relevant to costs. 
Figure~\ref{fig:alg} (c) illustrates the computation of a cost value for a single arc corresponding to an existing track at frame $k$ and a new detection at frame $k+1$.

We generate the cost matrix $c_{k+1}'$ using the base heuristic, which is described by four major components.
There is a set of motion models $M$, an object localization algorithm $Y$, an appearance model $A(\cdot)$, and a localization scoring function $L(\cdot)$.
Inductively, at time $k$, there exist a set of $m$ tracks.
We let $v^{(i,k')}$ denote a vector that represents an aggregation of appearance feature information until frame $k'$ for track $i$.
Moreover, each track $i$ is associated with a motion model $M_i$.
For each object $j$ at time $k+1$, the base heuristic will use $Y$ to generate a bounding box $B_{k+1}^j$.
Then, the motion model for each track $i$ will estimate the next state of $i$ via a new bounding box $B_{k+1}^i$ on frame $k+1$.
The base heuristic then (if applicable) generates an appearance score $A(v^{(i,k)},\bar{B}_{k+1}^j)$, where $\bar{B}_{k+1}^j$ denotes a representation of the image defined by bounding box $B_{k+1}^j$.
We then compute a localization score $L(B_{k+1}^i,B_{k+1}^j)$, which yields a spatial similarity measure.
The matrix $c_{k+1}'$ is then defined as
\begin{equation}\label{eq:initialmat}
    c_k'^{(ij)}=f(A(v^{(i,k)},\bar{B}_{k+1}^j),L(B_{k+1}^i,B_{k+1}^j)),
\end{equation}
where $f(\cdot)$ is a function defined by the base heuristic, and $c_{k+1}'^{(ij)}$ refers to the element of the $i^\text{th}$ row and $j^\text{th}$ column of $c_{k+1}'$.


We now explain how to generate matrix $c_{k+1}''$, which represents a cost matrix that aggregates appearance score information over time.
At a high level, we generate $c_{k+1}''$ by comparing each existing track at $k$ with the generated future tracklets, specifically those with their first detection as the detections from time $k+1$. 
We propose exploiting the previous frame features of the existing tracks by obtaining the appearance similarity between the past and the future frame features, which is intuitively and experimentally (confirmed in Appendix~\ref{appendix:ablationexp3}) a better measure to match an object that has re-appeared. 
For an object $j$ at frame $k+1$, we use the base heuristic to generate a tracklet $t_{k+1}^j$ that extends to time $k + \ell + 1$.
Note that these new tracklets are obtained from the simulation of the base heuristic using a reinitialized motion model at frame $k+1$.
At a high level, we will perform a pairwise comparison of tracklets generated by the base heuristic with existing tracks.
Suppose an object $j$ is mostly occluded over some time window.
Then in this time window, the appearance features of $j$ are less relevant since $j$ is not visible.
Let $v'^{(i)}$ be a $k$-dimensional vector, where each element $v'^{(i)}_{k'}$ is a real value indicating how informative the detection at frame $k'$ is to matching future detections for track $i$.
We generate $v'^{(i)}$ by appending appearance score $A(v^{(i,k)},\bar{B}_{k+1}^j)$ to $v'^{(i)}$ after each frame association to the $j^{\text{th}}$ object.
We refer to $v'^{(i)}$ as the \textit{appearance quality vector} for track $i$.
For each track/tracklet pair $i,t_{k+1}^j$, we begin at frame $k$ and search backward through $i$ until we find a time $k'$ where $v'^{(i)}_{k'}$ is below some threshold parameter $\tau$.
This represents a time in the past when the corresponding object is visible.
%In the case where no appearance feature smoothing is used, we may simply let $k'=k-1$. 
We then consider a limited window $W_i$ of $s$ frames in track $i$ beginning at time $k'-s+1$ and ending at $k'$.
We then compare each of the detections in $t_{k+1}^j$ with each of the detections in $W_i$.
We compare a detection $n$ of $t_{k+1}^j$ and a detection $n'$ of $W_i$ by independently calculating the appearance feature similarity score using appearance model $A$ on $n$ and $n'$.
Lastly, we obtain $c_{k+1}''^{(ij)}$ by taking an average across all pair-wise comparisons, i.e.
\begin{equation}\label{eq:prev_future_score}
    c_{k+1}''^{(ij)}=\frac{1}{s\cdot \ell}\sum_{n'\in W_i}\sum_{n\in t_{k+1}^j}A(n,n')
\end{equation}

In the final phase of ADPTrack, we compute the cost matrix $c_{k+1}$ as
\begin{equation}
    c_{k+1}=\alpha c_{k+1}''+(1-\alpha)c_{k+1}',
\end{equation}
where $0\le\alpha\le1$ is a user-selected weight parameter.
For performing association between frames $k+1$ and $k$ over the augmented cost matrix $c_{k+1}$, we apply the weighted bipartite matching scheme as prescribed by the base policy.
Lastly, if an object $j$ is matched to a track $i$, we then append $A(v^{(i,k)},\bar{B}_{k+1}^j)$ to $v'^{(i)}$ and continue to associate frames $k+1$ and $k+2$.
A pseudocode description of ADPTrack is presented in Algorithm~\ref{alg:adptrack}.

\begin{algorithm}
\caption{ADPTrack with Base Heuristic $H=(M,Y,A,L,f)$}
\label{alg:adptrack}
    \begin{algorithmic}[1]
    \Statex{\textbf{Parameters:} $\ell,s\in\mathbb{Z}^+$; $\tau\in\mathbb{R}^+$; $\alpha\in[0,1]$.}
    \Statex{\textbf{Input:} A set of $N+1$ frames; a set of $m$ tracks of length $k$; 
    a set of ($k$)-dimensional appearance quality vectors $\{v'^{(i)}\mid i\in\{1,\ldots,m\}\}$.}
    \Statex{\textbf{Output:} A set of $m$ tracks of length $k+1$; a set of $k+1$-dimensional appearance quality vectors $\{v'^{(i)}\mid i\in\{1,\ldots,m\}\}$.}
  
        \State{Initialize empty matrix $c_{k+1}'$.}
        \For{each track $i$} 
            \For{each object $j$ on frame $k+1$}
                \State{Generate bounding box $B_{k+1}^j$ with $Y$.}
                \State{Generate bounding box $B_{k+1}^i$ with $M_i$.}
                \State{Set $c_{k+1}'^{(ij)}\gets f(A(v^{(i,k)},\bar{B}_{k+1}^j),L(B_k^i,B_{k+1}^j))$.}
            \EndFor
        \EndFor
        
            \State{Perform data association over frames $k+1$ to $k + \ell + 1$ using $H$.}\label{alg:assoc}
            \State{Use output from Line~\ref{alg:assoc} to obtain tracklet $t_{k+1}^j$ for each object $j$ at frame $k+1$.}
        
        \State{Initialize empty matrix $c_{k+1}''$.}
        \For{each track $i$} 
            \State{Set $k'\gets \infty$.}
                
                    \For{$k''=k,k-1,\ldots,1$}
                        \If{$v'^{(i)}_{k''}<\tau$}
                            \State{Set $k'\gets k''$}
                            \State{\textbf{break}}
                        \EndIf
                    \EndFor   
        
             \If{$k'=\infty$}
                \State{Set $k'\gets k$}
              \EndIf
                \State{Set $W_i$ as set of frames $\max\{1,k'-s+1\}$ to $k'$.}
           
            \For{each object $j$ on frame $k+1$}
                \State{Set $c_{k+1}''^{(ij)}\gets\frac{1}{s\cdot \ell}\sum_{n'\in W_i}\sum_{n\in t_{k+1}^j}A(n,n')$.}
            \EndFor
        \EndFor
        \State{Set $c_{k+1}\gets \alpha c_{k+1}''+(1-\alpha)c_{k+1}'$.}\label{alg:skip}
        \State{Compute minimum weight bipartite matching $u_{k}$ on $c_{k+1}$.}
        \State{Append $u_{k}$ to track set.}

            \For{each $(i,j)\in u_{k}$}
                \State{Append $A(v^{(i,k)},\bar{B}_{k+1}^j)$ to end of $v'^{(i)}$.}
            \EndFor
    \end{algorithmic}
\end{algorithm}

*************************
Existing literature in MOT can be classified into four areas: offline, batch, online, and near-online tracking.


Offline tracking performs assignments considering all the frames of the video sequence~\cite{gogm, lifm, graphfusion, fusion, mht, mhtr, tlmht, edmt, bilstmmht}.


Batch tracking can be viewed as a special case of offline tracking where a limited number of frames are considered at once~\cite{multicut, dnf, famnet, gtt, mpntracker}.

In~\cite{asmot}, the authors formulate the multi-object tracking and segmentation problem as a dynamic programming problem. 


******************************************************************************
In particular, we present the procedure through which the weights $c_{k+1}^{ij}$ that forms value function approximations $\Tilde{J}_{k+1}$ of the form \eqref{eq:kplus1tilde} are computed. It involves computing tentative tracks based on the base heuristic, and computes 

*************************************************************************
(a) Visualization of approximation in value space applied to the multi-dimensional assignment problem. The red layers represent those included in partial groupings up to time $k$. The cost function approximation $\tilde{J}_{k+1}(\cdot)$ is dependent on a cost matrix $c_{k+1}$, which is computed using information obtained from a truncated horizon of length $\ell$ (blue and orange layers).
    We select a minimum weight perfect bipartite matching $u_k$ at time $k$ applied to $c_{k+1}$. (b) Visualization of near-online simulation in ADPTrack. A tracking simulation is performed for a truncated horizon ($\ell$ frames) using a base heuristic with a motion model. The base heuristic is initialized at time $k+1$ for the simulation. (c) Visualization of cost matrix approximation in ADPTrack. Consider the arc between the first track at frame $k$ and the second detection at frame $k+1$. To calculate the cost value $c^{12}_{k+1}$, unlike the base heuristic (online tracker) that compares the track at frame $k$ to the detection at frame $k+1$, we compare the track at frame $k$ to the tracklet starting at frame $k+1$ generated by the near-online simulation. The comparison is performed by pairwise appearance features similarity computations (Equation \ref{eq:prev_future_score}).

    % \subsection{Multi-dimensional assignment}
% In this section, we present Figure~\ref{fig:multidim} to aid the understanding of the literature presented in Section~\ref{multidim}.

% \begin{figure}
%     \centering
%     \includegraphics[width=.6\textwidth]{Styles/multidim.pdf}
%     \caption{Depiction of a 6-dimensional instance of the multi-dimensional assignment problem where $m=5$.
%      Green arcs represent the underlying arcs of the instance; red arcs define groupings. The solution is $m$ node-disjoint paths of length 6 where each path contains exactly one node from each layer (i.e. grouping).}
%     \label{fig:multidim}
% \end{figure}
